Resource-aware IoT Control: Saving Communication through Predictive Triggering

The Internet of Things (IoT) interconnects multiple physical devices in large-scale networks. When the 'things' coordinate decisions and act collectively on shared information, feedback is introduced between them. Multiple feedback loops are thus closed over a shared, general-purpose network. Traditional feedback control is unsuitable for design of IoT control because it relies on high-rate periodic communication and is ignorant of the shared network resource. Therefore, recent event-based estimation methods are applied herein for resource-aware IoT control allowing agents to decide online whether communication with other agents is needed, or not. While this can reduce network traffic significantly, a severe limitation of typical event-based approaches is the need for instantaneous triggering decisions that leave no time to reallocate freed resources (e.g., communication slots), which hence remain unused. To address this problem, novel predictive and self triggering protocols are proposed herein. From a unified Bayesian decision framework, two schemes are developed: self triggers that predict, at the current triggering instant, the next one; and predictive triggers that check at every time step, whether communication will be needed at a given prediction horizon. The suitability of these triggers for feedback control is demonstrated in hardware experiments on a cart-pole, and scalability is discussed with a multi-vehicle simulation.

==> content/6_TriggerAnalysis_old.tex <==
\section{Discussion}
% Analysis of triggers
\label{sec:analysisTriggers}
[This part has been significantly restructured, but most content kept.]

\medskip

In this section, we compare the obtained triggers, PT and ST, by analyzing their structure and discussing their triggering behavior through  numerical examples.  To focus on the essential triggering behavior and simplify the discussion, we consider the case without inputs ($B_i \vik{u}{i}{k-1} = 0$ in \eqref{eq:sys_x}).

In addition to the proposed triggers PT and ST, we also compare to an \emph{event trigger} (ET).
%We compare the proposed ST and PT to an event trigger (ET).  
Using the same framework developed herein,
% and considering the LTI case for simplicity, 
the ET can be obtained from the PT \eqref{eq:PTsquaredError1} by setting $M=0$:
%, which results in
\begin{align}
\gamma_{k} = 1 \,\, \Leftrightarrow \,\, 
\trigsig_{k|k}
%\E[  E_{k} | \Yall_k ] 
%= \norm{ \xKF_k - A^K \xP_\last  }^2 
&= \norm{ \xKF_k - A \xP_{k-1}  }^2  \label{eq:ETsquaredError} \\
&= \norm{ \xII_k - \xI_k  }^2\geq C_k. \nonumber
\end{align}
The trigger directly compares the two options at the remote estimator, $\xI_k$ and $\xII_k$.
%, with and without communication.
%the current local estimate to the remote estimate that results from not sending an update. 
To implement the ET, communication must be available instantaneously if needed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Trigger structure}

The derived rules for ST, PT, and ET have the same threshold structure
% Cut (for space constraints)
%\footnote{For the ST \eqref{eq:STsquaredError}, \eqref{eq:trigGenStructure} is understood in the sense that \eqref{eq:trigGenStructure} is evaluated for increasing $M\geq 1$ until a positive trigger $\gamma_{k+M}=1$ is found.} 
\begin{equation}
\gamma_{k+M} = 1 \,\, \Leftrightarrow \,\,  \trigsig_{k+M|k} \geq C_{k+M} 
\label{eq:trigGenStructure}
\end{equation}
where the communication cost $C_{k+M}$ corresponds to the triggering threshold.
The triggers differ in the expected estimation cost $\trigsig_{k+M|k}$. 
% We next analyze the structure of the triggers in more detail.
% , where we concentrate on the time-invariant case for simplicity. \todo{?}
To shed light on this difference, 
%For the purpose of comparing the structure of the different triggers, 
we introduce
\begin{align}
\trigsigM_{k,M} &:= \norm{ A^M (\xKF_k \! -\! A \xP_{k-1} ) }^2 \label{eq:trigSigMean} \\
\trigsigV_{k,M} &:= \trace( \PKF_{k+M|k} \!-\! \PKF_{k+M} ). \label{eq:trigSigVar}
\end{align}
With this, the triggers 
%We then have the following characterization:  the triggers 
ST \eqref{eq:STsquaredError}, PT \eqref{eq:PTsquaredError1}, \eqref{eq:PTsquaredError2}, and ET \eqref{eq:ETsquaredError} 
%can then be characterized as follows.  Each trigger is 
are given by \eqref{eq:trigGenStructure} with
\begin{align}
\trigsig_{k+0|k} &= \trigsigM_{k,0}, M=0 && \text{(ET)} \label{eq:ETcharacterization} \\
\trigsig_{k+M|k} &= \trigsigM_{k,M} + \trigsigV_{k,M} \quad \quad \quad && \text{(PT), $k > \lastel$} \label{eq:PTcharacterization1} \\
\trigsig_{k+M|k} &= \trigsigV_{\kappa,\Delta} && \text{(PT), $k \leq \lastel$} \label{eq:PTcharacterization2} \\
\trigsig_{\last+M|\last} &= \trigsigV_{\last,M} && \text{(ST)} . \label{eq:STcharacterization}
\end{align}
%
Hence, the trigger signals are generally a combination of the `mean' signal \eqref{eq:trigSigMean} and the `variance' signal \eqref{eq:trigSigVar}.  Noting that the mean signal \eqref{eq:trigSigMean} depends on real-time measurement data $\Yall_k$ (through $\xKF_k$), while the variance signal \eqref{eq:trigSigVar} does not, we can characterize ET and PT as 
%\emph{closed-loop}
\emph{online triggers}, while ST is an 
%\emph{open-loop}
\emph{offline trigger}. This reflects the intended design of the different
triggers. ST is designed to predict the next trigger at the time $\last$ of the
last triggering, without seeing any data beyond $\last$.  This allows the sensor
to go to sleep in-between triggers, for example.  ET and PT, on the other hand, continuously monitor the sensor data to make more informed transmit decisions (as shall be seen in the following comparisons).
%when comparing the effectiveness of the different triggers in the following examples).

While ET requires instantaneous communication, 
%which restricts online allocation of communication resources,
which is limiting for online allocation of communication resources,
%which is impractical  when integration with the communication system is desired, 
PT makes the transmit decision $M\geq1$ steps ahead of time.  ET compares the mean estimates only (\cf \eqref{eq:ETcharacterization}), while PT results in a combination of mean and variance signal (\cf \eqref{eq:PTcharacterization1}).  If a transmission is already scheduled for $\lastel_{k-1} \geq k$, PT resorts to the ST mechanism for predicting beyond $\lastel_{k-1}$; that is, it relies on the variance signal only (\cf \eqref{eq:PTcharacterization2}).
  
While ST can be understood as an \emph{open-loop} trigger (\eqref{eq:STcharacterization} can be computed without any measurement data), ET clearly is a \emph{closed-loop} trigger requiring real-time data $\Yall_k$ for the decision on $\gamma_k$.  PT can be regarded as an intermediate scheme exploiting real-time data and variance-based predictions.  
Accordingly, the novel predictive triggering concept lies between the known concepts of event and self triggering.

The ST is similar to the variance-based triggers proposed in \cite{TrDAn14b}.  
Therein, it was shown for a slightly different scenario (transmission of measurements instead of estimates) that event triggering decisions based on the variance are independent of any measurement data and can hence be computed off-line.
%For a slightly different scenario with transmission of measurements (instead of local estimates), it was shown therein that event triggering decisions based on the variance of the measurement prediction error are independent of any measurement data and can be computed off-line.  
Similarly, when assuming that all problem parameters $A$, $H$, $Q$, $R$ in \eqref{eq:sys_x}, \eqref{eq:sys_y} are known a-priori, 
%the variance signal \eqref{eq:trigSigVar} and thus 
\eqref{eq:STsquaredError} can be pre-computed for all times.  However, if some parameters only become available during operation (\eg the sensor accuracy $R_k$), the ST also becomes an online trigger. 
%In  \cite{TrDAn14b}, it was further shown that periodic transmit sequences result for variance-based triggering applied to a time-invariant process.
% \eqref{eq:sys_x}, \eqref{eq:sys_y}.
%  We shall also make this observation for the ST in the simulations in \sect \ref{sec:simulations}.

For the case with inputs ($B_i \vik{u}{i}{k-1} \neq 0$ in \eqref{eq:sys_x}), the triggering behavior is qualitatively similar.  The mean signal \eqref{eq:trigSigMean} will include the closed-loop dynamics $\bar{A}$ and the input $\xi_{k-1}$ corresponding to other agents, and the variance signal \eqref{eq:trigSigVar} will include the additional term $\Xi_{k,M}$ accounting for the additional uncertainty of not knowing the true input.
%Key characteristics of the proposed self-trigger (ST) and predictive trigger (PT) are illustrated through numerical simulations of stable and unstable scalar processes.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Behavior of self trigger}
%\subsection{Behavior of self and predictive triggers}
To illustrate the behavior of the ST, 
%First, 
we consider simulations of the stable, scalar, linear time-invariant (LTI) process:
\begin{example}
%System \eqref{eq:sys_x}, \eqref{eq:sys_y}, with 
$A = 0.98$, $H = 1$, $Q = 0.1$, $R = 0.1$, and $\bar{x}_0 = X_0 = 1$.
\label{ex:ex1}
\end{example}
%The results of the numerical simulation 
Results of the numerical simulation of the event-based estimation system (\cf \fig \ref{fig:remoteEstimation}) consisting of the local state estimator \eqref{eq:KF1}--\eqref{eq:KF5}, the remote state estimator \eqref{eq:remoteEst}, and the ST \eqref{eq:STsquaredError} with constant cost $C_k = C= 0.6$ are shown in \fig \ref{fig:example1_1}.
%
\begin{figure}[tb]
\centering
\includegraphics[scale=.88]{figure_example1_1}	% was 0.9
\caption{Example~\ref{ex:ex1} with self-trigger (ST).  
%The TOP graph shows the true state $x$ (\graph{black}), the KF estimate $\xKF$ (\graph{blue}), and the remote estimate $\hat{x}$ (\graph{orange}); and in the SECOND graph are the corresponding errors $\eKF=x-\xKF$ (\graph{blue}) and $e=x-\hat{x}$ (\graph{orange}).  
TOP: KF estimation error $\eKF=x-\xKF$ (\graph{blue}) and remote error $e=x-\hat{x}$ (\graph{orange}).
MIDDLE: 
%The THIRD graph shows 
components of the triggering signal 
$\trigsigM$ \eqref{eq:trigSigMean} (\graph{blue}), $\trigsigV$ \eqref{eq:trigSigVar} (\graph{orange}), the triggering signal $\trigsig = \trigsigM + \trigsigV$ (\graph{black}, hidden), and the threshold $C_k = 0.6$ (\graph{dashed}).  
BOTTOM: triggering decisions $\gamma$.
%The BOTTOM graph indicates the triggering decisions $\gamma$.
}
\label{fig:example1_1}
\end{figure}
The estimation errors of the local and remote estimator are
compared in the first graph.
As expected, the remote estimation error $e_k = x_k-\hat{x}_k$ (orange) is larger than the local estimation error $\eKF_k = x_k-\xKF_k$ (blue).  Yet, the remote estimator only needs 14\% of the samples.  

The triggering behavior is illustrated in the second graph showing the
triggering signals $\trigsigM$ \eqref{eq:trigSigMean}, $\trigsigV$ \eqref{eq:trigSigVar}, and $\trigsig = \trigsigM + \trigsigV$, and the bottom graph depicting the triggering decision $\gamma$.
%As can be seen from the third graph in \fig \ref{fig:example1_1}, 
Obviously, the ST entirely depends on the variance signal $\trigsigV$ (orange, identical with $\trigsig$ in black), while $\trigsigM = 0$ (blue).  This reflects the previous discussion about the ST being independent of online measurement data.  
The triggering behavior (the signal $\trigsig$ and the decisions $\gamma$) is actually  \emph{periodic}, which can be deduced as follows:
%Furthermore, it can be seen that the triggering signal and thus also the transmit decisions $\gamma_k$ are \emph{periodic}.  This can be deduced as follows: 
%From KF theory \cite{AnMo05}, 
the variance $\PKF_k$ of the KF \eqref{eq:KF1}--\eqref{eq:KF5} converges exponentially to a steady-state solution $\PKFss$, \cite{AnMo05}; hence, the triggering law \eqref{eq:STsquaredError} asymptotically becomes  
$\trace( \Vo^M(\PKFss) - \PKFss ) \geq C$ with $\Vo(X) := AXA^\transp + Q$,
% Cut (space):
%\begin{align}
%\trace( \Vo^M(\PKFss) - \PKFss ) \geq C, \quad  \Vo(X) := AXA^\transp + Q
%\label{eq:STsquaredErrorLTI_ex1}
%\end{align}
and \eqref{eq:STgeneral} thus has a unique 
%(time-invariant) 
solution $M$ corresponding to the period seen in \fig \ref{fig:example1_1}.  
%Moreover, the triggering decision becomes deterministic in the that it is independent of any real-time data and can be computed off-line.

Periodic transmit sequences are typical for variance-based triggering on time-invariant problems, which has also been found and formally proven for related scenarios in \cite{TrDAn14b,LeDeQu15}.  
%Obviously, there is no such periodic solution for a general time-varying process \eqref{eq:sys_x}, \eqref{eq:sys_y}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Behavior of predictive trigger}
The results of simulating \Ex \ref{ex:ex1}, now with 
%For the same example, \Ex \ref{ex:ex1}, the simulation results of the event-based estimation system with 
the PT \eqref{eq:PTsquaredError1}, \eqref{eq:PTsquaredError2}, and prediction horizon $M=2$, are presented in \fig \ref{fig:example1_2} for the cost $C_k = C = 0.6$, and in \fig \ref{fig:example1_3} for $C_k = C = 0.25$.  Albeit using the same trigger, the two simulations show fundamentally different triggering behavior: while the triggering signal $\trigsig$ and the decisions $\gamma$ in \fig \ref{fig:example1_2} are irregular, they are periodic in \fig \ref{fig:example1_3}.  
%
\begin{figure}[tb]
\centering
\includegraphics[scale=.88]{figure_example1_2}
\caption{Example~\ref{ex:ex1} with predictive trigger (PT) and $C_k = 0.6$.  Coloring of the signals is the same as in \fig \ref{fig:example1_1}.  The triggering behavior is \emph{stochastic}.
}
\label{fig:example1_2}
\end{figure}
%
\begin{figure}[tb]
\centering
\includegraphics[scale=.88]{figure_example1_3}
\caption{Example~\ref{ex:ex1} with predictive trigger (PT) and $C_k = 0.25$.  Coloring of the signals is the same as in \fig \ref{fig:example1_1}. The triggering behavior is \emph{periodic}.
}
\label{fig:example1_3}
\end{figure}

Apparently, the choice of the cost $C_k$ determines the different behavior of the PT.
%
For $C_k = 0.6$, the triggering decision depends on both, the mean signal $\trigsigM$ and the variance signal $\trigsigV$, as can be seen from \fig \ref{fig:example1_2} (third graph).
%From \fig \ref{fig:example1_2} (third graph), it can be seen that for $C_k = C = 0.6$, the triggering decision depends on both, the mean signal $\chi_\text{mean}$ and the variance signal $\chi_\text{var}$.  
Because $\trigsigM$ is based on real-time measurements,
% (through $\xKF_k$ in \eqref{eq:PTsquaredError1}), 
which are themselves random variables \eqref{eq:sys_y}, the triggering decision is a random variable.  
We also observe in \fig \ref{fig:example1_2} that the variance signal $\trigsigV$ is alone not sufficient to trigger  a communication.
% Cut (space): \footnote{After convergence of the local estimator variance $\PKF_k$, $\trigsigV$ corresponds to \eqref{eq:STsquaredErrorLTI_ex1}, which does not exceed the chosen $C_k$ for $M=2$ iterations.}
However, when lowering the cost of communication $C_k$ enough, the variance signal alone becomes sufficient to cause triggers.  Essentially, triggering then happens 
%the prediction 
according to \eqref{eq:PTsquaredError2} only, and  \eqref{eq:PTsquaredError1} becomes irrelevant.  Hence, the PT resorts to self triggering behavior for small enough communication cost $C_k$.  That is, the PT undergoes a phase transition for some value of $C_k$ from stochastic/online triggering to deterministic/offline triggering behavior.

%While, for a stationary LTI system with constant cost $C_k=C$, the self-trigger is deterministic\footnote{Deterministic in the sense that \eqref{eq:STsquaredErrorLTI_ex1}, which is independent of real-time data and can be computed off-line, fully determines the periodic triggering sequence.}  for all $C$,
%the predictive trigger undergoes a phase transition for some value of $C$ from stochastic/on-line triggering decision to deterministic/off-line behavior.






\subsection{Estimation versus communication trade-off}
Following the approach from \cite{TrCa15}, we evaluate the effectiveness of different triggers by comparing their trade-off curves of average estimation error $\Ec$ versus average communication $\Cc$ obtained from Monte Carlo simulations.  In addition to the ST \eqref{eq:STsquaredError} and the PT \eqref{eq:PTsquaredError1}, \eqref{eq:PTsquaredError2}, $M=2$, we also compare against the ET \eqref{eq:ETsquaredError}.  The latter is expected to yield the best trade-off because it makes the triggering decision at the latest possible time (ET decides at time $k$ about communication at time $k$).  
%Yet, ET assumes that communication is available instantaneously if needed, and otherwise wasted, which is often impractical as argued in the introduction.

%The estimation error $\Ec$ versus average communication $\Cc$ curves are obtained from Monte Carlo simulations.
The estimation error $\Ec$ is measured as the squared error $e_k^2$ averaged
over the simulation horizon (200 samples) and \num{50000} simulation runs. 
The average communication $\Cc$ is normalized such that $\Cc=1$ means
$\gamma_k=1$ for all $k$, and $\Cc=0$ means no communication (except for one
enforced trigger at $k=1$).
By varying the constant communication cost $C_k = C$ in a suitable range, an $\Ec$-vs-$\Cc$ curve is obtained, which represents the estimation/communication trade-off for a particular trigger.  The results 
%from simulations of 
for \Ex \ref{ex:ex1} are shown in \fig \ref{fig:example1_EvsC}.
\begin{figure}[tb]
\centering
\includegraphics[scale=0.9]{figure_example2_EvsC} % was: .9
\caption{Trade-off between estimation error $\Ec$ and average communication $\Cc$ for different triggering concepts applied to \Ex \ref{ex:ex1}. 
Each point represents the average from 50'000 Monte Carlo simulations, and the light error bars correspond to one standard deviation. 
%It can be seen that the novel concept of predictive triggering provides a middle ground between event triggering and self triggering. 
}
\label{fig:example1_EvsC}
\end{figure}

%Figure \ref{fig:example1_EvsC} compares the $\Ec$-vs-$\Cc$ curves for three different triggering concepts.
%In addition to the self trigger (ST) \eqref{eq:PTgeneral}, \eqref{eq:STsquaredErrorLTI} and the predictive trigger (PT) \eqref{eq:PTgeneral}, \eqref{eq:PTsquaredErrorLTI1}, \eqref{eq:PTsquaredErrorLTI2} with $M=2$, we also included simulations with an event trigger (ET).  The latter is obtained from \eqref{eq:PTsquaredErrorLTI1}, \eqref{eq:PTsquaredErrorLTI2} by setting $M=0$, which results in
%\begin{align}
%\E[  E_{k} | \Yall_k ] = \norm{ \xKF_k - A^K \xKF_\last  }^2 = \norm{ \xKF_k - A \hat{x}_{k-1}  }^2 .
% \label{eq:ETsquaredErrorLTI}
%\end{align}
%That is, the trigger compares the \emph{current} local to the remote estimate (in case no update is sent); it assumes that communication is available \emph{instantaneously} if needed.


Comparing the three different triggering schemes, we see that the ET is superior, as expected, because its curve is uniformly below the others.  Also expected, the ST is the least effective 
%in making the trade-off between estimation performance and communication requirements 
since no real-time information is available and triggers are purely based on variance predictions.  
%This makes perfect sense: the event-trigger can exploit the maximum available information for making a transmit decision (actually all data until and including the decision time), while the self-trigger decision is purely based on predictions.
% and thus incurs more uncertainty in the decision making.  
The novel concept of predictive triggering can be understood as an intermediate solution between these two extremes.  For small communication cost $C_k$ (and thus relatively large communication $\Cc$), the PT behaves like the ST, as was discussed in the previous section and is confirmed in \fig \ref{fig:example1_EvsC} (orange and black curves essentially identical for large $\Cc$).
%as discussed in the previous section and as can be seen in \fig \ref{fig:example1_EvsC} (orange and black curves identical for large $\Cc$).  
When the triggering threshold $C_k$ is relaxed (\ie the cost increased), the PT also exploits real-time data for the triggering decision (through \eqref{eq:trigSigMean}), similar to the ET.  Yet, the PT must predict the decision $M$ steps in advance making its $\Ec$-vs-$\Cc$ trade-off generally less effective than the ET.  In \fig \ref{fig:example1_EvsC}, the curve for PT is thus between ET and ST and approaches either one of them for small and large communication $\Cc$.
%; for small $\Cc$, it approaches the performance of ET, and for large $\Cc$, the performance of ST.  

% Cut (space):
%The same qualitative behavior of the different triggering mechanisms is observed for an unstable process; results can be found in \cite{Tr16}.

%Fig.\ \ref{fig:example2_EvsC} shows the $\Ec$-vs-$\Cc$ curves for the unstable system:
%\begin{example}
%%System \eqref{eq:sys_x}, \eqref{eq:sys_y}, with 
%$A_k = 1.1$, $H_k = 1$, $Q_k = 0.1$, $R_k = 0.1$ for all $k$, and $\bar{x}_0 = X_0 = 1$.
%\label{ex:ex2}
%\end{example}
%The same qualitative behavior of the different triggering mechanisms as in \fig \ref{fig:example1_EvsC} can be observed.
%\begin{figure}[tb]
%\centering
%\includegraphics[scale=0.98]{figure_example1_EvsC} % was: .9
%\caption{Estimation-vs-communication trade-offs for investigated triggering concepts applied to \Ex \ref{ex:ex2} (unstable process).
%}
%\label{fig:example2_EvsC}
%\end{figure}

